Connecting the Physical Properties of Galaxies with the Overdensity and Tidal Shear of the Large-Scale Environment

We have examined the correlations between the large-scale environment of galaxies and their physical properties, using a sample of 28,354 nearby galaxies drawn from the Sloan Digital Sky Survey, and the large-scale tidal field reconstructed in real space from the 2Mass Redshift Survey and smoothed over a radius of $\sim 6 h^{-1}$Mpc. The large-scale environment is expressed in terms of the overdensity, the ellipticity of the shear and the type of the large-scale structure. The physical properties analyzed include $r$-band absolute magnitude $M_{^{0.1}r}$, stellar mass $M_\ast$, $g-r$ colour, concentration parameter $R_{90}/R_{50}$ and surface stellar mass density $\mu_\ast$. Both luminosity and stellar mass are found to be statistically linked to the large-scale environment, regardless of how the environment is quantified. More luminous (massive) galaxies reside preferentially in the regions with higher densities, lower ellipticities and halo-like structures. At fixed luminosity, the large-scale overdensity depends strongly on parameters related to the recent star formation history, that is colour and D(4000), but is almost independent of the structural parameters $R_{90}/R_{50}$ and $\mu_\ast$. All the physical properties are statistically linked to the shear of the large-scale environment even when the large-scale density is constrained to a narrow range. This statistical link has been found to be most significant in the quasi-linear regions where the large-scale density approximates to an order of unity, but no longer significant in highly nonlinear regimes with $\delta_{\rm LS}\gg 1$.

==> makefile <==
SOURCE = ms

.SUFFIXES:	.aux .dvi .ps .tex

# edit and process the .tex file
default:	twice ps gv

main:		$(SOURCE).aux
			latex $(SOURCE)
dvi:		$(SOURCE).dvi
ps:			$(SOURCE).ps
once:
			latex $(SOURCE)
twice:		once once
			latex $(SOURCE)
bib:		
			bibtex $(SOURCE)

x:			$(SOURCE).dvi
			xdvi -geometry +0+0 -s 8 -bg white -fg black \
			-expert -hush $(SOURCE).dvi &
gv:			$(SOURCE).ps
			gv $(SOURCE).ps &


.dvi.ps:
			dvips -f $< > $(SOURCE).ps
.tex.aux:
			latex $(SOURCE)	# create .aux file from $<
.tex.dvi:
			latex $<	# create .dvi file from $<

clean:	
			rm -f *~ *.log *.dvi *.aux *.blg  *.lof *.lot *.toc *~ 
cleanest:	
			rm -f *~ *.log *.dvi *.ps *.aux *.toc


